Mining Weighted Sequential Patterns in Incremental Uncertain Databases

Due to the rapid development of science and technology, the importance of imprecise, noisy, and uncertain data is increasing at an exponential rate. Thus, mining patterns in uncertain databases have drawn the attention of researchers. Moreover, frequent sequences of items from these databases need to be discovered for meaningful knowledge with great impact. In many real cases, weights of items and patterns are introduced to find interesting sequences as a measure of importance. Hence, a constraint of weight needs to be handled while mining sequential patterns. Besides, due to the dynamic nature of databases, mining important information has become more challenging. Instead of mining patterns from scratch after each increment, incremental mining algorithms utilize previously mined information to update the result immediately. Several algorithms exist to mine frequent patterns and weighted sequences from incremental databases. However, these algorithms are confined to mine the precise ones. Therefore, we have developed an algorithm to mine frequent sequences in an uncertain database in this work. Furthermore, we have proposed two new techniques for mining when the database is incremental. Extensive experiments have been conducted for performance evaluation. The analysis showed the efficiency of our proposed framework.

==> Figures/figure_code.tex <==
\begin{figure}[htb]
    \centering % <-- added
\begin{subfigure}{0.45\linewidth}
  \includegraphics[width=\linewidth]{example-image-a}
  \caption{image1}
  \label{fig:1}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.45\linewidth}
  \includegraphics[width=\linewidth]{example-image-b}
  \caption{image2}
  \label{fig:2}
\end{subfigure}
% \hfil % <-- added
% \begin{subfigure}{0.25\textwidth}
%   \includegraphics[width=\linewidth]{example-image-c}
%   \caption{image3}
%   \label{fig:3}
% \end{subfigure}

\medskip
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{example-image-a}
  \caption{image4}
  \label{fig:4}
\end{subfigure}\hfil % <-- added
\begin{subfigure}{0.45\textwidth}
  \includegraphics[width=\linewidth]{example-image-b}
  \caption{image5}
  \label{fig:5}
\end{subfigure}
% \hfil % <-- added
% \begin{subfigure}{0.25\textwidth}
%   \includegraphics[width=\linewidth]{example-image-c}
%   \caption{image6}
%   \label{fig:6}
% \end{subfigure}
\caption{Fasi del processo di impregnazione}
\label{fig:images}
\end{figure}
